Appliance Operation Modes Identification Using Cycles Clustering

The increasing cost, energy demand, and environmental issues has led many researchers to find approaches for energy monitoring, and hence energy conservation. The emerging technologies of Internet of Things (IoT) and Machine Learning (ML) deliver techniques that have the potential to efficiently conserve energy and improve the utilization of energy consumption. Smart Home Energy Management Systems (SHEMSs) have the potential to contribute in energy conservation through the application of Demand Response (DR) in the residential sector. In this paper, we propose appliances Operation Modes Identification using Cycles Clustering (OMICC) which is SHEMS fundamental approach that utilizes the sensed residential disaggregated power consumption in supporting DR by providing consumers the opportunity to select lighter appliance operation modes. The cycles of the Single Usage Profile (SUP) of an appliance are extracted and reformed into features in terms of clusters of cycles. These features are then used to identify the operation mode used in every occurrence using K-Nearest Neighbors (KNN). Operation modes identification is considered a basis for many potential smart DR applications within SHEMS towards the consumers or the suppliers

==> tex/DTW.tex <==

%todo---------------------------------------------------------------------------------------------
\section{Single Use Profile Classification With DTW}
\label{dtw} 
For each time that the appliance has been activated we need to determine the appliance operation mode. This requires a comparison of the time series at the point that the appliance has been activated and the reference patterns for each of the operational modes. We describe the approach using Dynamic Time Warping (DTW) \cite{ratanamahatana2004everything} .

%=============================================
\subsection{Day Consumption Segmentation}
Let us assume that  an appliance runs in $ n $ operation modes denoted by the set $  M = \{m_1,m_2,...,m_n\} $.  The daily consumption is represented by $ D(t) $ which  contains subsequences  representing appliance usages.  For each mode $ m_i $  the reference pattern is represented by $ P^{m_i}(t) $  where $k^{m_i}$ is the SUP size of operation mode $ m_i $. A segment $ G^{m_i}(t)$ is a sub-sequence of the daily consumption function $ D(t) $, starting from the point of the turn on time $t_{on}$ and with the size $k^{m_i}$ representing the size of operation mode $m_i$. This is defined as follows:
\begin{equation} \label{eq:dtw03}
G^{m_i}(t) = D(x) \quad : \quad x \in [t_{on} , t_{on}+k^{m_i}]
\end{equation}

\noindent for each reference pattern, $ P^{m_i}(t)$, for an operation mode $ m_i $ and turn on time $t_{on}$, segments of the daily consumption, D(t) can be extracted using Eq.\ref{eq:dtw03}.

The segmentation is visually presented in Figure.\ref{fig:dtwSegmenter}. In part (a) $ D(t) $ is shown, and the segmentation starting point is indicated by the vertical dashed line at $t_{on}$. The segment sizes are highlighted in different shades so that each shade corresponds to the size of the segment for a specific operation mode. Part (b) shows the generated reference functions   $ P^{m_i}(t) $ that are used to specify segments sizes $ \{k^{m_1},k^{m_2},..,k^{m_n}\} $. Lastly, in part (c) the segment functions $ G^{m_i}(t)$ are listed.
	\begin{figure}
	\centering
	\includegraphics[width=.47\textwidth]{images/ch6/dtwSegmenter}
	\caption{ Visual representation of the segmentation and applying DTW.}
	\label{fig:dtwSegmenter}
	\end{figure}
%=============================================
\subsection{Classification of SUPs Based On DTW Distances}
The DTW algorithm \cite{ratanamahatana2004everything} uses two inputs which are the two functions $ G^{m_i}(t)$ and $ P^{m_i}(t) $ representing sequences. It then performs a calculation to find the distance (or similarity) between these two functions as the output. Figure.\ref{fig:dtwSegmenter} shows the inputs and the outputs of the DTW algorithm. The DTW is invoked $ n $ times where $ n $ equals the number of RPs representing operation modes for an appliance. For each reference pattern and the corresponding segment, the distance is calculated. Let X denote the sequence represented by $ P^{m_i}(t) $ and let Y represent the sequence  $ G^{m_i}(t)$.  The DTW distance is formulated as follows:

\begin{equation} \label{eq:dtw05}
\begin{array}{l}
d_i = \mathrm{DTW}(X,Y )
\\
M=\{m_1,..,m_i, ... m_n\}
\end{array}
\end{equation}

The value of the distance calculated by DTW is inversely proportional to the similarity.  Thus we assume that the most similar reference pattern is the reference pattern with the minimum distance. This means that the mode $m^*$ with the minimum distance $d^*$ that is the operation mode of the appliance at the SUP detected at $t_{on}$ as:
\begin{equation*} \label{eq:dtw06}
\begin{array}{l}
d^* = min (d_1,	d_2,	...,	d_{m_i})
\end{array}
\end{equation*}

==> tex/analysis_short.tex <==

\section{Power Consumption Data Analysis}
\label{analysis} 
We use Power Consumption Datasets (PCDs) to understand the power consumption characteristics of appliances over time when turned on. 
We focused on the analysis of The Rainforest Automation Energy dataset (RAE) \cite{Makonin2017} and the work done by Pipattanasomporn et.al. \cite{Pipattanasomporn2014} where demand response opportunities were provided for some household appliances. In this paper, the appliances data that we analyzed are the clothes washer, clothes dryer, and dishwasher. 
%=============================================
\subsection{Single Usage Profile}
A Single Usage Profile (SUP) is used to formally characterize power consumption of an appliance between the time it is turned on and the time it is turned off.  The analysis of the datasets is presented in \ref{analysisAppliances}  and is used to determine SUPs.
Single Usage Profile (SUP) represents the sequence of power consumption values consumed by an appliance from the moment of turning it on to the moment of that it is turned off. Hence, SUP with the sampling frequency $f_s=1Hz$  is defined by the sequence $\{ p_i \}_{i=t_{on}}^{t_{off}}$ where $p_i$ is the instantaneous power reading at time $i$. The times $t_{on}, t_{off}$ is the turn on, turn off times respectively of the appliance and $i \in [t_{on}, t_{off}]$ represents the $i^{th}$ sample. Figure \ref{fig:Washwe_uses_powers_h2} shows multiple SUPs for a clothes washer over the course of around two months.

%=============================================
\subsection{The Analysis Of Appliances Power Consumption}
\label{analysisAppliances} 
The SUP for the dishwasher is shown in Figure \ref{fig:Dishwasher_All_modes}. The dishwasher has three main operating modes: Heavy, Medium, and Light. Each SUP of the dishwasher has three states: Wash, Rinse and Dry, regardless of the operation mode. For example, in the Light mode, the first 70 minutes are associated with the wash state. The rinse state follows from minutes 70 to 97. The last state is the drying state which ends at minute 108.
	\begin{figure}
	\centering
	\fbox{\includegraphics[trim={1.7cm 1.7cm 1.7cm 1.7cm },clip,width=.47\textwidth]{images/ch3/Dishwasher_All_modes}}
	\caption{Single Usage Profile (SUP) for the dishwasher showing three operation modes: (a) Heavy, (b) Medium, (c) Light.}
	\label{fig:Dishwasher_All_modes}
	\end{figure}

The same type of analysis is performed for the clothes washer and the clothes dryer. The clothes washer has three states that occur for each single use: wash, rinse, and spin, sorted in ascending order of power consumption level.  A single operation of the clothes dryer uses three states with different temperatures: Maximum Heat, Medium Heat, No Heat. During the Maximum Heat state the dryer drum is heated to the maximum temperature in the dryer setting, and so on for the other states. 

By analyzing appliances data, we found similar patterns. Each activation with certain operation mode has a specific pattern of consumption based on the states of the appliance. These states are preconfigured by the manufacturer in terms of timing and power consumption levels.


==> tex/detection.tex <==

%todo---------------------------------------------------------------------------------------------
\section{Single Use Profile Detection}
\label{detection} 
With Demand Response,  consumers are encouraged to use appliances in off peak hours. This requires the need to detect when appliances are activated. Hence, we can advice the user to shift the load or not based on the detected time. This serves as a basis for further analysis in determining appliance operation modes.

%=============================================
\subsection{The Reference Pattern}
We use a Reference Pattern (RP) which represents the start of a SUP. RP is a sequence of data points represented as $ S(t) $ which returns the data point that represents the power value associated with $ t $. We focus on matching RP to a subsequence of the daily time series which is represented by $ D(t) $. RP is derived from a generated SUP by taking a slice of the generated SUP corresponding to turning on the appliance.
%=============================================
\subsection{Cross Correlation}
In time series analysis, Cross Correlation (XCORR) \cite{MENKE2016187} is a measure of similarity of two series as a function of the displacement of one series relative to the other series. Assume two time series represented by $ f(t) $ where $ t \in [1,n]$ and $ g(t) $ where $  t \in [1,m] $ and $ n < m $. Assuming that the number of moving windows is finite, the XCORR function, $ X(t) $, for $ f(t) $ with $  g(t) $ is defined as follows:
   	\begin{equation} \label{eq:det02}
		X(t)= (f\star g)(t)\ = \sum _{k=1 }^{n }f(k)g(t+k)
	\end{equation}
To avoid calculations with large numbers, we use another option by using the absolute difference instead of multiplication. If we use the absolute difference, the  XCORR function $X(t)$ between $S(t)$ and $D(t)$  is the following: 
	\begin{equation} \label{eq:det04}
	X(t)= (S\star D)(t)\ = \sum _{k=1 }^{n }\Big| S(k) - D(t+k)\Big| \quad,\quad t\in[1,m-n]
	\end{equation}
\noindent where $ m $ represents the number of daily samples in $ D(t) $ and $ n $ is the number of samples used in $ S(t) $.

A normalization step takes place to invert $X(t)$ over the y-axis by subtracting all correlation values from the average of the maximum power value for both  $S(t)$ and $D(t)$. This normalization makes the similarity between the two functions relative to their maximum values. Therefore, the two functions are more similar when the normalized correlation value is closer to the average of maximum values found in the sequences represented by $ S(t) $ and $ D(t) $. The normalized cross correlation function $ X(t)  $ is the following:
	\begin{equation} \label{eq:det05}
	X(t) = \frac{Max(S(t)) + Max(D(t))}{2} - \frac{1}{n} \sum _{k=1 }^{n }\Big| S(k) - D(t+k)\Big| \quad,
	\end{equation}
	\[
		\quad t\in[1,m-n]
	\]
	\begin{figure}
	\centering
	\includegraphics[width=.47\textwidth]{images/ch5/xcorr}
	\caption{ The reference pattern represented by the function $ S(t) $. The cross correlation plot $ X(t) $ and the day consumption function $ D(t) $ over the day time. }
	\label{fig:detxcorr}
	\end{figure}
Figure.\ref{fig:detxcorr} shows a graphical depiction of the XCORR function $ X(t) = (S\star D)(t)$.
$ S(t) $ is shown in Figure.\ref{fig:detxcorr}. RP shows $ 600 $ samples in this case. $ X(t) $ is shown in Figure.\ref{fig:detxcorr} . The fluctuation in the value of $ X(t) $ starts around 8:50 PM as illustrated in Figure.\ref{fig:detxcorr} (b) which depicts a zoomed in view for the period 8:45 PM to 9:45 PM. These fluctuations represent the overlap between the two correlated functions. Higher values of $X(t)$  means that there is more overlap present between the functions and therefore, higher similarity. $X(t)$ shows its maximum value at approximately 9:00 PM, which means that the potential SUP starts at this time. The turn on time of the appliance in $D(t)$ is observed at 9:00 PM as seen in  Figure.\ref{fig:detxcorr} (b) representing the maximum value of $X(t)$.
%=============================================
\subsection{Determining Turn On Times}
 
We use X(t) to determine the potential turn on times. It is not feasible to consider all times at the local maximums of $X(t)$ as potential turn on times since $D(t)$ could contain multiple periods where there is not a considerable level of similarity with the reference pattern. Also, the noise contained within the correlation function may cause local maximums even after a smoothing function is applied. To overcome these problems we introduce a Low Amplitude Canceling Coefficient $\delta$ that limits the range of where to look for the local maximums. The role of the $\delta$ coefficient is to cancel out all values of $ X(t) $ that is lower than a threshold $\tau$ determined by $\delta$, so that the residue function $\overline{X}(t)$ of $X(t)$  after applying $\delta$ represents all periods that contain the local maximums that is greater than $\tau$. The value of $\delta$ is selected with the assumption that $ \delta \in (0,1) $. $\overline{X}(t)$ is defined as the following:
	\begin{equation} \label{eq:det07}
	\overline{X}(t) = X(t) - \tau
	\end{equation}
\noindent where the value of the threshold $\tau$ is calculated as follows:
	\begin{equation} \label{eq:det06}
	\tau = \delta \;  \frac{Max(S(t)) + Max(D(t))}{2} \quad ,\quad \delta \in (0,1)
	\end{equation}
Figure.\ref{fig:detCancel} (b) shows the plot of  $ \overline{X}(t) $. Since $ \overline{X}(t) $ is a trimmed version of $ X(t) $ where  $ X(t) $ is thresholded by $\tau$ value to produce $ \overline{X}(t) $, then $ \overline{X}(t) $ is zero except for short periods of time. These periods of time are what remained from $ X(t) $ after applying the threshold $\tau$. $ \overline{X}(t) $ contains isolated periods of time where the value of the correlation is relatively the highest among the entire period of the day. The shape of the $ \overline{X}(t) $ is a group of continuous concave down curves that resembles the highest values of $ X(t) $ where $X(t) > \tau$. Therefore, the position of the potential turn on time would be at the absolute maximum of each of these concave down curves. These periods in Figure.\ref{fig:detCancel} are $p_1, p_2$ where $p_1=[ p_1^{start} , p_1^{end}]$ and $p_2=[ p_2^{start} , p_2^{end}]$ . These periods have their own absolute maximum values at $p_1^{max}, p_2^{max}$ respectively within their domains. This maximum value represents the highest value of the cross correlation at this period, which means that the time when this maximum values occur is a potential turn on time. Consequently, the absolute maximum in $p_1$ is $X_1^{max}$ at $t= p_1^{max}$, and the absolute maximum in $p_2$ is $X_2^{max}$ at $t= p_2^{max}$. We then conclude that $\{p_1^{max}, p_2^{max}\} $ is the set of the potential turn on times. 

\begin{figure}
	\centering
	\includegraphics[width=.47\textwidth]{images/ch5/detCancel}
	\caption{\textbf{(a)} The positioning of the threshold $\tau$ relative to the residue function $ \overline{X}(t) $. \textbf{(b)} A zoomed in version of $ \overline{X}(t) $. The plot shows the absolute maximum $X_i^{max}$ for each tip of spike  $i$ enclosed in the period $p_i=[ p_i^{start} , p_i^{end}]$ }
	\label{fig:detCancel}
\end{figure}

==> tex/results_short.tex <==

%todo---------------------------------------------------------------------------------------------
\section{Results And Discussion}
\label{results}
\begin{figure}
	\centering
	\includegraphics[width=.48\textwidth]{images/ch9/allNumSUP}
	\caption{The impact of changing the reference pattern size $n$ on the number of detected SUPs in the day consumption date for a dishwasher, a clothes washer, and a clothes dryer. }
	\label{fig:allNumSUP}
\end{figure}
This section discusses the results of applying SUP detection using XCORR and SUP classification using DTW and KNN on test data.
\subsection{Single Usage Profile Detection}
The evaluation metric we use is \textit{the number of detected SUPs } for certain appliance. This corresponds to the number of reported turn on times for certain appliance by the SUP detection algorithm.  We assume that a single SUP presents daily for an appliance. We generated reference patterns of different sizes $n$ based on a SUP generated with a randomly selected operation mode  (see \cref{simulation}).  We assume that the value of the Low Amplitude Canceling Coefficient $\delta$ is equal to 90 and the sampling frequency used is $f_s = 1Hz$.

Figure.\ref{fig:allNumSUP} shows the results for a dishwasher, a clothes washer, and a clothes dryer. For the dishwasher, it shows a very large number of detected SUPs found in the day when n is between 50 and 400. This is because of the shape of the SUP of the dishwasher. When the reference pattern size is  between 50 and 400, there is a high number of SUPs detected despite the existence of only one SUP. However, the number of detected SUP settles down to one when the reference pattern size typically increases within the range 400 and 1400 samples. When the reference pattern size exceeds 1400 samples, the number of detected SUPs is zero.
For the clothes washer. When the reference pattern size is between 100 and 1100 samples, the number of detected potential SUPs is always one. That is probably because the repetition in the washer consumption curve is minimal, thus, a unique one high value of cross correlation in every test.
For the clothes dryer, it shows that the value of $n$ that gives best results is when $n$ is between 600 and 1100 samples where it shows the number of detected SUPs equals to one. Nevertheless, the results show some choppiness in the number of detected SUPs. This is a common problem for all appliances. It is most likely due to the variations in cycles duration where cycle duration is generated with variation factor that affects XCORR by reducing the overlapping between the cycles in the reference pattern and the detected SUP.

The number of matching SUPs is higher for shorter reference pattern than a longer reference pattern. This is because there is higher chance that small reference pattern occurs more frequently within the consumption function than a longer reference pattern. The reason is that a SUP has repetitions of cycles that have similar shape. This shape could be similar to the reference pattern. This leads to reporting multiple potential SUPs even where is only one SUP. Thus, as the size of reference pattern decreases, the probability of reporting these repetitions within a SUP is higher. Therefore, the accuracy increases as the reference pattern size increases. 

\subsection{Single Usage Profile Classification}
	\begin{figure}
		\centering
		\includegraphics[width=.48\textwidth]{images/ch9/DTWbox}
		\caption{The precision, recall and F1-score for each operation mode using DTW. }
		\label{fig:DTWbox}
	\end{figure}

To test the performance of the DTW classifier, we generate power consumption data for three different households using the simulator.  These datasets are distinct in appliance usage in terms of $I_h$. We assume that for each appliance, there are three different levels of $I_h$: High, Medium, and Low.

We use three metrics to measure the performance of the classifiers we use. The metrics are the following: Precision, Recall, F1-score. Figure.\ref{fig:DTWbox} shows that for the DTW the metrics values are averaged around 82\% for the light and heavy operation modes. Otherwise, the metrics value is approximately 79\%.

The breakdown of the operation modes performance for each appliance  is shown in Figure.\ref{fig:evalAll2}. The chart is divided into three main lanes, each lane corresponds to an appliance. Within each lane, it shows the different metric values for DTW classification results over the operation modes. Generally, the chart shows higher performance for the light and heavy operation modes. In the clothes washer lane, there is a variation in the metrics values from operation mode to another. However, in the clothes dryer and the dishwasher lanes,it shows higher performance for heavy and light modes more noticeably in the clothes dryer.


==> tex/simulator.tex <==
\section{POWER CONSUMPTION SIMULATION}
\label{simulator}
It is sometimes necessary to create simulated data when it is impractical to obtain real data that may have protected information, may not be available for legal reasons or there is an insufficient amount of data \cite{Dickert2011}. Therefore, simulated datasets have the potential to provide the sufficient data needed to evaluate algorithms.  
use of sensors in houses that monitor disaggregated power consumption.  This makes it difficult to evaluate algorithms used to make recommendations on reducing power consumption. This section focuses on developing a simulator for generating Synthetic Power Consumption DataSets (SPCDSs).
The publicly available power consumption datasets (PCDSs) are scarce \cite{Pipattanasomporn2014,pflugradt2013analysing} and often limited to aggregated power consumption of a residence with minimal information specific to each appliance. However, when the appliance specific information is available, there is a lack of diversity of usage patterns for the same appliance over a long period of time and the different operation modes for an appliance are not captured. These limitations are due to the limited 

The main objective of the Power Consumption Simulator (PCS) is to generate PCDSs that mimic the publicly available PCDSs. PCS generates daily power consumption for certain appliance in certain household. PCS generates Synthetic Single Usage Profiles (SSUPs) that simulate the behavior of the SUPs of the appliance analyzed in public PCDSs with multiple operation modes. PCS also simulates the probabilistic timing on when each SSUP occurs within the day and distribution of operation modes for each SSUP.

\subsection{Simulator Parameters}
The simulator is controlled by the following parameters: Turn on times distribution which represent the time of the day that an appliance is activated by the user. The second parameter is the Household Usage Intensity distribution which refers to the pattern of operation modes that a household selects over time. The third parameter is the SUP Representation Object (SUPRO) which is a JSON object that contains a formal representation for any SUP.

\subsubsection{ Turn On Time Distribution}
\label{TurnOnTime}
Turn on time ($t_{on}$) distribution refers to the time when an appliance is activated by the user during the day. We use the Inverse Transform Sampling (ITS) \cite{miller2010inverse} method to sample values of $t_{on}$.
The probability of turning on appliance, $ a $, at time, $ t $, is represented by  $ f_T^a(t) $ such that:
\begin{equation} \label{eq:sim01}
f_T^a(t) = Pr(T=t) \quad , \quad t\in D
\end{equation}
where D is a set of discrete time partitions that represents one day. For example, if the day is partitioned into 24 hours then $D= \{0,1,2,...,23\}$.


The next step is to compute the Cumulative Distribution Function (CDF), $F_T^a(t)$, as follows:
\begin{equation} \label{eq:sim02}
F_T^a(t_x) = \sum_{t=0}^{t\in D, t\leq t_x} f_T^a(t)
\end{equation}

ITS uses the CDF as the basis for sampling random values of turn on times.


\subsubsection{ Household Usage Intensity Distribution}
\label{sec:Intensity}
Household Usage Intensity distribution refers to the distribution of operation modes that a household uses over time. It takes the values: Low, Medium, and High. The operation mode that is used more frequently than the others is called the\textit{ Major Operation Mode}, while other less frequently used operation modes are the\textit{ Minor Operation Modes}.
Households are considered as \textbf{high intensity}in their usage when they use an appliance in heavy operation mode more than using it with the light or medium operation modes, so in this case the major operation mode is the heavy mode. Also, households are considered as \textbf{medium intensity} when they use an appliance in medium operation mode more than using it with heavy and light operation modes, so in this case the major operation mode is the medium mode. Finally, households are considered as \textbf{low intensity} when they use an appliance in light operation mode more than using it with heavy and medium operation modes, so in this case the major operation mode is the light mode.  For example, let us consider a household with medium usage intensity that uses a dishwasher for a month. This household uses the medium operation mode (major) for the dishwasher most of the time, e.g., let's say 60\% of the time e.g., 18 days. The light and heavy modes (minor) are used 20\% of the time each e.g., 6 days each.

We assume that the selection of an appliance mode for a household is based on a multinomial distribution function. The frequencies of this distribution is as follows:
\[ 
\mathrm{operation \; mode}  = 
\begin{cases} 
minor  &,  20\% \\
major  &, 60\% \\
minor  &, 20\% 
\end{cases}
\]

The major mode occupies the highest frequency since the household will use this mode most of the time. The minor modes are selected a fewer number of times. 


ITS is used to select an operation mode.The mode is selected based on the value of $i_h$ which is sampled from a multinomial distribution function with the the aforementioned frequencies. By selecting these values the majority of the samples (60\%) will be selected from the major mode, while each of the other two minor modes will be selected with lower chance.



\subsubsection{SUP Representation Object}
The \textit{SUP Representation Object} (SUPRO) is a JSON representation of a SUP in a particular operation mode. This is used by the simulator to generate SSUPs based on the representation contained in SUPROs.

\cref{fig:Dryer_all_modes2}  shows three SUPs for a clothes dryer corresponding to  three different operation modes. The clothes dryer has three different cycles within each single use: No Heat, Half Heat, Max Heat. These cycles are characterized by their time, duration, and power consumption level. These cycles are also repeated through the duration of the usage by either singularly (such as the max heat cycle) or in pairs (such as the no heat followed by the half heat). The duration of each occurrence of a cycle changes e.g., for the no heat cycle, all the occurrences have a 3 to 4 minute duration except the last no heat cycle which runs for over 8 minutes. Also, the repetition of pairs of cycles differs among operation modes. For example, Half Heat and No Heat cycles in the heavy mode are repeated 22 times per phase. However, in the medium operation mode there are 19 repetitions.

 The following is the description of the attributes contained in a SUPRO:
\begin{enumerate}
	\item \textbf{Appliance:} This attribute is used to specify the appliance.
	
	\item \textbf{Operation Mode:} This attribute is used to specify the operation mode.
	
	\item \textbf{Phases:}{ This is an array where each element is a phase. Each phase in this array contains the following attributes:
		\begin{enumerate}
			\item \textbf{Repeat Minimum:} This is used to determine the lower bound of the number of repetitions of the phase.
			
			\item \textbf{Repeat Maximum:} This is used to determine the upper bound of the number of repetitions of the phase. The number of repetitions is selected randomly between the lower and upper bounds.
			
			\item \textbf{Cycles:}{ This is an array where each element is a cycle. Each cycle in this array contains the following attributes:
				
				\begin{enumerate}
					\item \textbf{Name:} This is used to determine the name of the cycle.
					
					\item \textbf{Power:} This attribute represents the average power value (amplitude) of this cycle.
					
					\item \textbf{Duration:} This attribute represents the duration of the cycle in seconds. 
				\end{enumerate} 
			}
		\end{enumerate} 
	}	
\end{enumerate} 

\begin{figure}[t]
	\centering
	\includegraphics[width=1.5in]{images/simConfigJSONall2}
	\caption{A snippet of SUP Representation Object (SUPRO).}
	\label{fig:simConfigJSONall}
\end{figure}

A graphical depiction of the SUP representation object structure is presented in \cref{fig:simConfigJSONall} where a SUP consists of multiple phases, illustrated as blue boxes. Each phase is duplicated one or more times based on the lower (Repeat Minimum) and upper bounds (Repeat Maximum) e.g., phase-1 occurred a single time while phase-2 is repeated multiple times. The reason behind introducing these two bounds is that the number of repetitions varies among models for the same appliance type. The use of lower and upper bounds can be used by the simulator to provide more realistic data that reflects the variation among different manufacturers.


\subsection{SSUP Generator}
This section describes the approach used to generating a day of consumption data and the process of generating a single SSUP, how the phases are repeated, and how the cycles are generated.

\subsubsection{SSUP Phases Simulation}
In the SUPRO, each phase is associated with a lower bound (RepeatMin) and an upper bound (RepeatMax).  The number of repetitions of a phase is based on the selection of random value  in the interval $ [RepeatMin, RepeatMax] $ such that:
\[
\textit{\mbox{Number of Repetitions} }= rnd(RepeatMin,RepeatMax)
\]

\subsubsection{SSUP Cycles Simulation}
To simulate a cycle of an appliance, we \textbf{first} calculate the simulated cycle power value, $ p_{sim}$ using the equation:
\begin{equation} \label{eq:sim07}
p_{sim} =  (1+ \alpha) p_{rep}\quad,\quad \alpha \in (0,1]
\end{equation}  
\noindent where $ p_{rep} $ is the power value of the cycle in the SUPRO. A noise component is added to the power value to make the power value more realistic in terms of randomness. $ p_{sim} $ is the power value after adding the noise element and $\alpha$ is the Cycle Power Variation Coefficient which is selected within the interval $[-1,1]$. The value of $\alpha$ is chosen based on a normal distribution with the assumption that $ \mu = 0, \sigma=0.2 $ so that the variation values are mostly focused around the power value in the SUP representation $ p_{rep} $. Also, since $\alpha \in [-1,1]$, the power variation could be positive or negative, so the simulated power value  $ p_{sim} $ could be more, less, or equal to the power values in the representation  $ p_{rep} $ .

The \textbf{second} parameter that controls the shape of the cycle is the Duration Variation Coefficient $\beta$, which changes the duration of the simulated cycle proportional to the value in the SUPRO as the equation:

\begin{equation} \label{eq:sim08}
d_{sim} =  (1+ \beta) d_{rep}, \beta \in (0,1]
\end{equation} 
where $d_{rep}$ is the cycle duration configured in the SUPRO while $d_{sim}$ is the simulated duration value. The value of $\beta$ is obtained from a normal distribution function with  $ \mu = 0, \sigma=0.2$. 

\IncMargin{1em}
\begin{algorithm}
	\caption{getSUP()}
	\label{alg:getSUP}
	\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	\Input{SUP Representation Object (SUPRO)}
	\Output{Synthetic Single Usage Profile (SSUP)}
	\BlankLine
	
	rep = getSUPRO().getOperationMode() \;
	SUPpower = [] \;
	\For{$i = 0 $ \KwTo $size(rep.phases)-1$}{
		repeat = randomBetween(rep.repeatMin,rep.repeatMax) \;
		\For{$j = 0 $ \KwTo $repeat-1$}{
			PhasePowers = [] \;
			\For{$k = 0 $ \KwTo $size(config.phases[i].cycles)-1$}{
				duration = rep.phases[i].cycles[k].duration*(1+ $\beta$ ) \;
				\For{$l = 1 $ \KwTo $duration$}{
					power = rep.phases[i].cycles[k].power*(1+ $\alpha$ )\;
					PhasePowers.add(power) \;
				}
			}
			SUPpower.addRange(PhasePowers) \;
		}
	}
	return SUPpower\; 
\end{algorithm}
\DecMargin{1em}  

The Simulator uses Algorithm \ref{alg:getSUP} to generate synthetic SUPs. The inputs of the algorithm is the SUP Representation Object for an appliance. The output is a synthetic SUP for the specified appliance for the specified mode.  
Lines 1 and 2 initialize the mode of the appliance and the array that stores the power values of the synthetic SUP. 
Lines 3 to 16 is repeated for each phase in the SUP representation object. 
Line 4 specifies the number of phases to iterate over within the variation limits specified  in the SUP representation object.
Lines 5 to 14 is repeated for all cycles in a phase. 
Line 6 initializes the array that holds the power values of the current phase. 
Lines 7 to 13 iterate over all cycles in the current phase. 
Line 8 calculates the duration (as number of samples) of the cycle based on the input representation and the variation coefficient. 
Lines 9 to 12 loop over every randomly generated power value in the current cycle to simulate. 
Lines 10 and 11 calculate the randomly generated power value and add this value into the phase power array. 
Line 14 joins the synthetic SUP power array with the current phase power array.


\subsection{Simulator Architecture}
\cref{fig:simModel} depicts the architecture of the simulator used with the inputs and outputs. The SUP Representation Object is used to shape the simulated consumption data for a single usage. The turn on time distribution is used determine the timing of which the activation of each appliance take place. The Household Usage Intensity distribution is used to determine the household the majority of the operation modes used over time. Tuning parameters are also provided to the simulator to add variation and stochasticity to the output. These parameters are the following: Cycle Power Variation Coefficient ($\alpha$), Duration Variation Coefficient ($\beta$), Turn Off Noise Coefficient ($\gamma$), and the Smoother Window Size $k$. The output of the simulator represents a simulated power consumption data for a single appliance in a single day.

%%motivation
Basically, the SUP Representation Object is passed to the SUP Generator to generate a new synthetic SUP. A smoothing function is applied to the synthetic SUP to cancel out unwanted high frequency noise. Finally, turn on time $t_{on}$, household intensity $i_h$, and the smoothed SSUP are passed to the One Day Generator. In this module a group of turn on times and operation modes are generated based on each SUP Representation Object. A new synthetic SUP is generated and placed at the corresponding  $t_{on}$. This represents the power consumption for a single day for a particular appliance. 


\begin{figure}[t]
	\centering
	\includegraphics[width=3.5in]{images/simModel}
	\caption{The Power Consumption Simulator architecture, inputs, and outputs.}
	\label{fig:simModel}
\end{figure}

%%the effect of the tuning params
The number of synthetic SUPs is determined by the number of sampled $t_{on}$ times through the day. The time of each synthetic SUP is determined by the generated $t_{on}$ value. Also, the operation mode of the synthetic SUP is defined by the sampled mode from the household intensity distribution. lastly, the tuning parameters affect timing $t_{on}$, power amplitude and the noise outside the synthetic SUP. 


\subsection{Generating Daily Power Consumption}
This section describes the generation of synthetic data for an appliance for one day.  
This is accomplished in the following steps: 
\textbf{First}, the turn on times and operation modes are generated using the ITS technique that is described in \cref{TurnOnTime} and \cref{sec:Intensity}.
\textbf{Second}, the generation of the SSUPs depends on the representation object that is selected based on the operation mode determined in the previous step.
\textbf{Third}, the idle power values between SSUPs is generated. These values correspond to the time between SUPs that represents the rest of the day time when the appliance is turned off or idle \cite{Alcala2016, Papaioannou2017} . These periods of time are represented by random low amplitude noise that correspond to low consumption components of the appliance such as LEDs, displays, etc. This noise is generated randomly and is tuned by Idle Noise Coefficient $\gamma$ which is assumed to take values such that $\gamma \in (0,40) $ W. 

\IncMargin{1em}
\begin{algorithm}
	\caption{generateDayPowerConsumption()}
	\label{alg:getDayPowerUsage}
	\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	\Input{Turn on times distribution $(t_{on})$, Usage Intensity distribution, and SUP Representation Object (SUPRO)}
	\Output{One day of power usage for an appliance}
	\BlankLine
	$t_{on} = $ getRandomTurnOnTime() \;
	mode = getRandomIntensity()\;
	dayPowers = [] \;
	SSUP  = getSUP(SUPRO)//Alg.1\;
	\For{$j = 1 $ \KwTo $t_{on}$}{
		dayPowers.add(randomBetween(0,$\gamma$))\;
	}
	dayPowers.addRange(SSUP)\;
	\For{$size(SUP) + t_{on} $ \KwTo $ DayEnd $}{
		dayPowers.add(randomBetween(0,$\gamma$))\;
	}
	return dayPowers \;
\end{algorithm}
\DecMargin{1em}


Algorithm \ref{alg:getDayPowerUsage} is used to generate one day of power usage with the presence of a single synthetic SUP within this day for simplicity. The inputs of the algorithm are the following: Turn on times distribution, Usage Intensity distribution, and SUP Representation Object. The output is simulated power consumption for a certain appliance for a single day.
Lines 1 and 2 initialize $t_{on}$, and the synthetic SUP operation mode using the techniques described in \cref{TurnOnTime} and \cref{sec:Intensity}.
Line 3 initializes the power array with the number of samples of the day. This array stores the power values for the whole day. 
Line 4 generates a new synthetic SUP with the generated operation mode from line 2.
Lines 5 to 7 generate random power noise values before the appliance is turned on.
Line 8 appends the synthetic SUP power values to the day power values at the specified turn on time.
Lines 9 to 11 generate random power noise values after the appliance is turned on.

==> tex/simulator_short.tex <==

%todo---------------------------------------------------------------------------------------------
\section{Power Consumption Simulation}
\label{simulation} 
It is necessary to create simulated data when it is impractical to obtain real data that there is an insufficient amount of certain type data such as our case when there is no such PCD that contains disaggregated data with different operation modes for an appliance. Our Power Consumption Simulator (PCS) main purpose is to simulate appliances consumption with different operation modes by generating daily usage data that has SUPs for different operation modes.

PCS has three configuration parameters: Turn On Time $t_{on}$, Household Usage Intensity ($I_h$), and SUP Representation Object (SUPRO). $t_{on}$ refers to the time when an appliance, \textit{a}, is activated by the user during the day. We use the Inverse Transform Sampling (ITS) \cite{miller2010inverse} method to sample values of $t_{on}$ Probability Density Function (PDF) that is extracted from a PCD. Household Usage Intensity ($I^a_h$) refers to the distribution of operation modes that a household, \textit{h}, uses for an appliance, \textit{a}, over time.  We assume that the selection of an appliance operation mode for a household is based on a multinomial distribution function. The frequencies of this distribution is 20\% for operation modes used fewer number of times and 60\% for the operation modes used more. Single Usage Profile Re presentation Object (SUPRO)  is a representational model of a SUP for an appliance in a particular operation mode.  It defines \textit{Cycles} which are periods of time when the power consumption is stable around fixed wattage. Each cycle is defined by the duration and the wattage it has. Also, SUPRO defines \textit{Phases} which are groups of cycles in certain repetition bounded by lower and upper bounds.


